Left/Right Hand Segmentation in Egocentric Videos

Wearable cameras allow people to record their daily activities from a user-centered (First Person Vision) perspective. Due to their favorable location, wearable cameras frequently capture the hands of the user, and may thus represent a promising user-machine interaction tool for different applications. Existent First Person Vision methods handle hand segmentation as a background-foreground problem, ignoring two important facts: i) hands are not a single "skin-like" moving element, but a pair of interacting cooperative entities, ii) close hand interactions may lead to hand-to-hand occlusions and, as a consequence, create a single hand-like segment. These facts complicate a proper understanding of hand movements and interactions. Our approach extends traditional background-foreground strategies, by including a hand-identification step (left-right) based on a Maxwell distribution of angle and position. Hand-to-hand occlusions are addressed by exploiting temporal superpixels. The experimental results show that, in addition to a reliable left/right hand-segmentation, our approach considerably improves the traditional background-foreground hand-segmentation.

==> tables/elliptic_similarity.tex <==
\begin{table}[h!]
\centering
    \caption{Left and right hand identification at contour level} \label{tab:maskidentification}
    \todo[inline,color=white]{To answe this we would need to define the distance between two ellipses}
% Table generated by Excel2LaTeX from sheet 'similarity of ellipses'
\begin{tabular}{rrrrrrr}
\toprule
     & \multicolumn{1}{c}{\begin{sideways}Coffe\end{sideways}} & \multicolumn{1}{c}{\begin{sideways}CofHoney\end{sideways}} & \multicolumn{1}{c}{\begin{sideways}Hotdog\end{sideways}} & \multicolumn{1}{c}{\begin{sideways}Pealette\end{sideways}} & \multicolumn{1}{c}{\begin{sideways}Tea\end{sideways}} & \multicolumn{1}{c}{\begin{sideways}Total\end{sideways}} \\
\midrule
\multicolumn{1}{c}{Left} &      &      &      &      &      &  \\
\multicolumn{1}{c}{Right} &      &      &      &      &      &  \\
\bottomrule
\end{tabular}%


\end{table}


==> tables/leftRight_givenHands.tex <==
\begin{table}[h!]
\centering
\caption{Evaluation of the hand segmentation only when split is required and given that the hand-segmenter already detect the pixel as hand-like} \label{tab:occlusion}
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{tabular}{rrr}
\toprule
         & Left    &   Right     \\
\midrule
Left     & 0.990   &   0.009\\
Right    & 0.006   &   0.993\\
\bottomrule
\end{tabular}%
\end{table}


==> tables/segmentation_identification.tex <==
\begin{table}[h!]
\scriptsize
\centering
    \caption{Left and right hand identification at a pixel level after segmentation. This table only considers frames without occulusions} \label{tab:pixellevelidentification}
    \todo[inline,color=white]{This table requires some code and i dont want to modify to much the code while the experiment in apolo finish to select the parameters}
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{tabular}{rrrr|rrr}
\toprule
        & \multicolumn{3}{c|}{No-Competition}  &  \multicolumn{3}{c}{With-Competition} \\
\midrule
        & No-Hand & Left & Right & No-Hand & Left & Right \\
\midrule
No-Hand &         &      &       &         &      &   \\
Left    &         &      &       &         &      &   \\
Right   &         &      &       &         &      &   \\
\bottomrule
\end{tabular}%
\end{table}

